Quantum Error Correction in Quaternionic Hilbert Spaces

We propose quaternion-based strategies for quantum error correction by extending quantum mechanics into quaternionic Hilbert spaces. Building on the properties of quaternionic quantum states, we define quaternionic analogues of Pauli operators and quantum gates, ensuring inner product preservation and Hilbert space conditions. A simple encoding scheme maps logical qubits into quaternionic systems, introducing natural redundancy and enhanced resilience against noise. We construct a quaternionic extension of the five-qubit code, introducing a framework of 15 syndrome measurements to detect quaternionic errors, including quaternionically rotated error components. Numerical estimates show that the quaternionic five-qubit code achieves a logical error threshold of approximately $p_{th} \approx 0.015$, demonstrating improved performance compared to the standard complex-valued code. These results suggest a new pathway for quantum error correction in high-noise environments, leveraging the richer structure of quaternionic quantum mechanics to improve fault tolerance.

==> references.tex <==
@book{adler1995quaternionic,
  title={Quaternionic quantum mechanics and quantum fields},
  author={Adler, Stephen L},
  volume={88},
  year={1995},
  publisher={Oxford University Press}
}
@article{arbab2010quaternionic,
  title={The quaternionic quantum mechanics},
  author={Arbab, Arbab I},
  journal={arXiv preprint arXiv:1003.0075},
  year={2010}
}
@article{danielewski2020foundations,
  title={Foundations of the quaternion quantum mechanics},
  author={Danielewski, Marek and Sapa, Lucjan},
  journal={Entropy},
  volume={22},
  number={12},
  pages={1424},
  year={2020},
  publisher={MDPI}
}

@article{birkhoff1936logic,
  title={The logic of quantum mechanics},
  author={Birkhoff, Garrett and von Neumann, John},
  journal={Annals of Mathematics},
  volume={37},
  number={4},
  pages={823--843},
  year={1936}
}
@article{yang1950,
  author = {Yang, C. N.},
  title = {On Quantized Space-Time},
  journal = {Physical Review},
  volume = {72},
  number = {9},
  pages = {874--874},
  year = {1950}
}
@book{home1997conceptual,
  author    = {Dipankar Home},
  title     = {Conceptual Foundations of Quantum Physics: An Overview from Modern Perspectives},
  publisher = {Plenum Press},
  address   = {New York, NY, USA},
  year      = {1997}
}
@book{voight2021quaternion,
  title={Quaternion algebras},
  author={Voight, John},
  year={2021},
  publisher={Springer Nature}
}
@article{hamilton1843new,
  title={On a new species of imaginary quantities, connected with the theory of quaternions},
  author={Hamilton, William Rowan},
  journal={Proceedings of the Royal Irish Academy (1836-1869)},
  volume={2},
  pages={424--434},
  year={1840},
  publisher={JSTOR}
}
@article{val1964homographies,
  title={Homographies, quaternions and rotations},
  author={Val, Du},
  journal={(No Title)},
  year={1964}
}
@article{bluvstein2024logical,
  title={Logical quantum processor based on reconfigurable atom arrays},
  author={Bluvstein, Dolev and Evered, Simon J and Geim, Alexandra A and Li, Sophie H and Zhou, Hengyun and Manovitz, Tom and Ebadi, Sepehr and Cain, Madelyn and Kalinowski, Marcin and Hangleiter, Dominik and others},
  journal={Nature},
  volume={626},
  number={7997},
  pages={58--65},
  year={2024},
  publisher={Nature Publishing Group UK London}
}
@article{acharya2024quantum,
  title={Quantum error correction below the surface code threshold},
  author={Acharya, Rajeev and Abanin, Dmitry A and Aghababaie-Beni, Laleh and Aleiner, Igor and Andersen, Trond I and Ansmann, Markus and Arute, Frank and Arya, Kunal and Asfaw, Abraham and Astrakhantsev, Nikita and others},
  journal={Nature},
  year={2024}
}
@article{aoki2009quantum,
  title={Quantum error correction beyond qubits},
  author={Aoki, Takao and Takahashi, Go and Kajiya, Tadashi and Yoshikawa, Jun-ichi and Braunstein, Samuel L and Van Loock, Peter and Furusawa, Akira},
  journal={Nature Physics},
  volume={5},
  number={8},
  pages={541--546},
  year={2009},
  publisher={Nature Publishing Group UK London}
}
@article{alder1986quaternionic,
  title={Quaternionic quantum field theory},
  author={Alder, Stephen L},
  journal={Communications in Mathematical Physics},
  volume={104},
  pages={611--656},
  year={1986},
  publisher={Springer}
}
 @misc{ enwiki:1284950161,
    author = "{Wikipedia contributors}",
    title = "Quaternion --- {Wikipedia}{,} The Free Encyclopedia",
    year = "2025",
    url = "https://en.wikipedia.org/w/index.php?title=Quaternion&oldid=1284950161",
    note = "[Online; accessed 24-April-2025]"
  }
@article{fowler2012surface,
  title={Surface codes: Towards practical large-scale quantum computation},
  author={Fowler, Austin G and Mariantoni, Matteo and Martinis, John M and Cleland, Andrew N},
  journal={Physical Review A—Atomic, Molecular, and Optical Physics},
  volume={86},
  number={3},
  pages={032324},
  year={2012},
  publisher={APS}
}
@article{steane1998introduction,
  title={Introduction to quantum error correction},
  author={Steane, AM},
  journal={Philosophical Transactions of the Royal Society of London. Series A: Mathematical, Physical and Engineering Sciences},
  volume={356},
  number={1743},
  pages={1739--1758},
  year={1998},
  publisher={The Royal Society}
}
@article{devitt2013quantum,
  title={Quantum error correction for beginners},
  author={Devitt, Simon J and Munro, William J and Nemoto, Kae},
  journal={Reports on Progress in Physics},
  volume={76},
  number={7},
  pages={076001},
  year={2013},
  publisher={IOP Publishing}
}
@article{dennis2002topological,
  title={Topological quantum memory},
  author={Dennis, Eric and Kitaev, Alexei and Landahl, Andrew and Preskill, John},
  journal={Journal of Mathematical Physics},
  volume={43},
  number={9},
  pages={4452--4505},
  year={2002},
  publisher={American Institute of Physics}
}
@article{kitaev2003fault,
  title={Fault-tolerant quantum computation by anyons},
  author={Kitaev, A Yu},
  journal={Annals of physics},
  volume={303},
  number={1},
  pages={2--30},
  year={2003},
  publisher={Elsevier}
}
@article{fowler2009high,
  title={High-threshold universal quantum computation on the surface code},
  author={Fowler, Austin G and Stephens, Ashley M and Groszkowski, Peter},
  journal={Physical Review A—Atomic, Molecular, and Optical Physics},
  volume={80},
  number={5},
  pages={052312},
  year={2009},
  publisher={APS}
}
@article{takagi2017error,
  title={Error rates and resource overheads of encoded three-qubit gates},
  author={Takagi, Ryuji and Yoder, Theodore J and Chuang, Isaac L},
  journal={Physical Review A},
  volume={96},
  number={4},
  pages={042302},
  year={2017},
  publisher={APS}
}
@article{bennett1996mixed,
  title={Mixed-state entanglement and quantum error correction},
  author={Bennett, Charles H and DiVincenzo, David P and Smolin, John A and Wootters, William K},
  journal={Physical Review A},
  volume={54},
  number={5},
  pages={3824},
  year={1996},
  publisher={APS}
}
@article{laflamme1996perfect,
  title={Perfect quantum error correcting code},
  author={Laflamme, Raymond and Miquel, Cesar and Paz, Juan Pablo and Zurek, Wojciech Hubert},
  journal={Physical Review Letters},
  volume={77},
  number={1},
  pages={198},
  year={1996},
  publisher={APS}
}
@article{yoder2016universal,
  title={Universal fault-tolerant gates on concatenated stabilizer codes},
  author={Yoder, Theodore J and Takagi, Ryuji and Chuang, Isaac L},
  journal={Physical Review X},
  volume={6},
  number={3},
  pages={031039},
  year={2016},
  publisher={APS}
}
@article{wootton2012high,
  title={High threshold error correction for the surface code},
  author={Wootton, James R and Loss, Daniel},
  journal={Physical review letters},
  volume={109},
  number={16},
  pages={160503},
  year={2012},
  publisher={APS}
}
@article{bombin2012strong,
  title={Strong resilience of topological codes to depolarization},
  author={Bombin, H{\'e}ctor and Andrist, Ruben S and Ohzeki, Masayuki and Katzgraber, Helmut G and Martin-Delgado, Miguel A},
  journal={Physical Review X},
  volume={2},
  number={2},
  pages={021004},
  year={2012},
  publisher={APS}
}
@article{ohzeki2012error,
  title={Error threshold estimates for surface code with loss of qubits},
  author={Ohzeki, Masayuki},
  journal={Physical Review A—Atomic, Molecular, and Optical Physics},
  volume={85},
  number={6},
  pages={060301},
  year={2012},
  publisher={APS}
}
@article{vlasov1999error,
  title={Error correction with euclidean qubits},
  author={Vlasov, Alexander Yu},
  journal={arXiv preprint quant-ph/9911074},
  year={1999}
}
